Team Formation for Scheduling Educational Material in Massive Online Classes

Whether teaching in a classroom or a Massive Online Open Course it is crucial to present the material in a way that benefits the audience as a whole. We identify two important tasks to solve towards this objective, 1 group students so that they can maximally benefit from peer interaction and 2 find an optimal schedule of the educational material for each group. Thus, in this paper, we solve the problem of team formation and content scheduling for education. Given a time frame d, a set of students S with their required need to learn different activities T and given k as the number of desired groups, we study the problem of finding k group of students. The goal is to teach students within time frame d such that their potential for learning is maximized and find the best schedule for each group. We show this problem to be NP-hard and develop a polynomial algorithm for it. We show our algorithm to be effective both on synthetic as well as a real data set. For our experiments, we use real data on students' grades in a Computer Science department. As part of our contribution, we release a semi-synthetic dataset that mimics the properties of the real data.

==> discussion.tex <==
In the introduction to section~\ref{sec:group} we mentioned that our goal is to find a partition of students into groups, so that the group schedules benefit the individual students the most possible. We now show, that the objective of \maxbenefit\ achieves just that.


Observe, that in Equation~\ref{eq:partitionP} the benefit of every student $s$ is computed with regard to the schedule $\calA_P$. If $\calA_P = \schedule(P,d)$, then this schedule is optimal for the group $P$. However, it may be that for the individual student $s$ this is not the optimal schedule. Let $\calA_s = \schedule(\{s\},d)$  be the optimal schedule for $s$. Observe, that $\bB(\{s\},\calA_s)$ is the best possible result that $s$ can achieve with an individual schedule. We refer to this value as the \emph{potential} of $s$. However, if $s$ is part of group $P$,  then it may very well happen, that $\dU(s,d) = \bB(\{s\},\calA_s)- \bB(\{s\},\calA_P)> 0$, thus $s$ does not reach his full potential in this group. We borrow the notation $\dU(s)$ from physics and call this the \emph{potential difference} of $s$.

We can see that the smaller the potential difference for student $s$ is, the more he benefits from his groups' schedule. Hence, we define the \minpotential\ problem~\ref{prob:mpotential} as that of finding groups, so that the total potential difference over every group is minimized. 
\begin{problem}[\minpotential\ (\minp) ]\label{prob:mpotential}
Let $\bS$ be a set of  students and $\bT$ be  a set of topics. 
For every $s \in \bS$ and $t \in \bT$ let $\req(s,t)$ be the requirement of $s$ on $t$ and given for every student-topic pair. Find a partition \calP\ of students into $K$ groups, such that 
 \[\dU(\calP,d) = \sum_{P \in \calP} \sum_{s \in P}\dU(s,d)\]
 is minimized.  
\end{problem}

We now show that minimizing the potential difference (that results in highest individual benefit for students) is equivalent to maximizing the group benefits.

\begin{proposition}\label{prop:maxbenminpot}
 \maxbenefit\ (Prob.~\ref{prob:maxbenefit}) and \minpotential\ (Prob.~\ref{prob:mpotential}) are equivalent.
\end{proposition}
\begin{proof}
The first part in $\dU(\calP,d)$ is independent of the partition because $\sum_{P \in \calP}\sum_{s \in P}\bB(\{s\},\calA_s) = \sum_{is \in \bS}\bB(\{s\}, \calA_s)$.  Hence, minimizing the potential difference is equivalent to minimizing the second part, which is $ \sum_{P \in \calP} \sum_{s \in P} - \bB(\{s\}\calA_P)$. This on its turn is equivalent to maximizing its negative, which is the \maxbenefit\ objective.
\end{proof}




==> problem.tex <==
 Let $\bS = \{s_1,s_2,\ldots,s_n\}$ be a set of students and $\bT = \{t_1,t_2,\ldots,t_m\}$ be a set of topics. We assign topics to $d$ timeslots based on two very simple rules; only one topic can be assigned to each
timeslot but the same topic can appear in multiple slots.  A \emph{schedule} \calA\ is a collision free assignment of topics to the timeslots. \calA\ can be thought of as an ordered list of (possible multiple occurrences) of the topics.  For a topic $t \in \bT$ the tuple $\langle t,i \rangle$ denotes the $i^{th}$ occurrence of $t$ in a schedule. The notation $\calA[r] = \langle t,i\rangle$ refers to the tuple $\langle t, i \rangle$ that is assigned to timeslot $r$ in $\calA$. 


\mpara{Topic requirements.} For every student $s \in \bS$ and topic $t \in \bT$ there is a number of times that $s$ has to hear about $t$ in order for $s$ to learn every aspect of this topic. We call this number the \emph{requirement} of $s$ on $t$ and denote it by the integer function $\req(s,t)$. 
%We assume that until $s$ has met his requirements, there is a benefit for him every time he is educated about $t$. However, after $\req(s,t)$ repetitions of $t$, while there is no detriment, there is also no additional benefit for $s$.


\mpara{Benefits from topic.} In order for a student $s$ to be fully knowledgeable about topic $t$, he has a requirement to learn $\req(s,t)$ times about $t$. We assume that until $s$ has met his requirements,  he  gains  knowledge and hence, will benefit to some extent from every repetition of $t$. After $\req(s,t)$ repetitions of $t$, while there is no detriment, there is also no additional benefit to $s$ from hearing about $t$.
We call $\bb(s,\langle t,i\rangle)$  (Equation~\eqref{eq:benefitdef}) the \emph{benefit} of $s$ from topic $t$ when hearing about it for the $i^{th}$ time. We assume that $s$ benefits equally from each of the first $\req(s,t)$ occurrences of $t$ in \calA, thus $\bb(s,\langle t,i\rangle) = \frac{1}{\req(s,t)}$ if $i \leq \req(s,t)$. Since after this point $s$ has already mastered topic $t$, there is no additional benefit from any later repetition of $t$ and hence  $\bb(s,\langle t,i\rangle) = 0$.
 \begin{equation}\label{eq:benefitdef}
 \bb(s,\langle t,i\rangle) =
  \begin{cases}
   \frac{1}{\req(s.t)} & \text{if\ } i\leq \req(s,t) \\
   0       & \text{otherwise}
  \end{cases}
\end{equation}
We note, that for ease of exposition we assume that all repetitions of $t$ before $\req(s,t)$ carry equal benefit to $s$. But, the definition and all of our later algorithms could easily be extended to use some other function $\bb'(s,\langle t,i\rangle)$. A natural choice for example is a function, where earlier repetitions of $t$ carry higher benefit than later ones, thus $\bb'(s,\langle t,i\rangle) = \frac{1}{2^i}$. The intuition is, that first you learn about the fundamentals of $t$ and later you add on additional information.
 
 
 Given the benefits $\bb(s,\langle t,i\rangle)$  there is a natural extension to define the benefit $\bB(s,\calA)$ that $s$ has from schedule \calA. This benefit is simple a sum over all timeslots in \calA,
 \begin{equation}\label{eq:benefit}
 \bB(s,\calA) = \sum_{r =1}^d\bb(s,\calA[r])
 \end{equation}
 Remember, that in Equation~\eqref{eq:benefit} $\calA[r]$ refers to the tuple $\langle t ,i \rangle$ that is scheduled at timeslot $r$ in \calA.
 
 
Observe, that every time topic $t$ appears in the schedule \calA,
it will contribute with the same amount of benefit towards
$\bB(s,\calA)$, regardless of the exact timeslot allocation
within  \calA. The order in which topics  are
scheduled will be important when there is one  schedule catered towards
multiple students at the same time as opposed to individual student schedules. We discuss this in detail in the next Section~\ref{sec:group}. 

\mpara{Scheduling constraints.} In real-life, most often we cannot pick any scheduling of topics we like. Instead, there are strict precedence constraints among the topics. For example, one has to learn addition before he can learn about multiplication during a math course. For this reason, we assume that along with the topics, a set of constraints is given. The constraints can be simple ones, such as the first occurrence of topic $t_i$ has to be before topic $t_j$. Or more complicated ones, topic $t_j$ can only be scheduled after at least $r_1$ repetitions of $t_{i_1}$ and $r_2$ repetitions of $t_{i_2}$. Of course, the set of constraints can also be empty, if we do not have any of them.

